GenDeg: Diffusion-based Degradation Synthesis for Generalizable All-In-One Image Restoration

Deep learning-based models for All-In-One Image Restoration (AIOR) have achieved significant advancements in recent years. However, their practical applicability is limited by poor generalization to samples outside the training distribution. This limitation arises primarily from insufficient diversity in degradation variations and scenes within existing datasets, resulting in inadequate representations of real-world scenarios. Additionally, capturing large-scale real-world paired data for degradations such as haze, low-light, and raindrops is often cumbersome and sometimes infeasible. In this paper, we leverage the generative capabilities of latent diffusion models to synthesize high-quality degraded images from their clean counterparts. Specifically, we introduce GenDeg, a degradation and intensity-aware conditional diffusion model capable of producing diverse degradation patterns on clean images. Using GenDeg, we synthesize over 550k samples across six degradation types: haze, rain, snow, motion blur, low-light, and raindrops. These generated samples are integrated with existing datasets to form the GenDS dataset, comprising over 750k samples. Our experiments reveal that image restoration models trained on the GenDS dataset exhibit significant improvements in out-of-distribution performance compared to those trained solely on existing datasets. Furthermore, we provide comprehensive analyses on implications of diffusion model-based synthetic degradations for AIOR.

==> sec/5_ablations.tex <==
\section{Ablations and analysis}


\newcolumntype{C}{>{\centering\arraybackslash}X}

\begin{table*}[t]
    \centering
    \caption{Performance Comparison of Various Methods on Different Datasets}
    \small
    \label{tab:performance_comparison}
    \begin{tabularx}{\textwidth}{l *{9}{C}}  % 'l' for Method, 'C' for others
        \toprule
        \textbf{Method} & 
        \textbf{REVIDE (R)} & 
        \textbf{O-Haze (R)} & 
        \textbf{RainDS (S)} & 
        \textbf{LHP (R)} & 
        \textbf{RSVD (S)} & 
        \textbf{GoPro (R)} & 
        \textbf{LOLv1 (R)} & 
        \textbf{SICE (R)} & 
        \textbf{RainDS (R)} \\
        \midrule
        DiffUIR & 
        0.268/58.5 & 
        0.334/147.2 & 
        0.088/31.2 & 
        0.187/26.5 & 
        0.176/26.1 & 
        0.144/25.2 & 
        0.148/65.1 & 
        0.442/102.9 & 
        - \\
        
        Diff-Plugin & 
        0.281/72.9 & 
        0.377/164.7 & 
        0.194/45.0 & 
        0.178/30.2 & 
        0.207/22.5 & 
        0.217/32.8 & 
        0.195/70.5 & 
        0.233/69.2 & 
        - \\
        
        InstructIR & 
        0.313/65.4 & 
        0.341/154.5 & 
        0.117/29.2 & 
        0.139/21.2 & 
        - & 
        0.146/21.1 & 
        0.132/57.3 & 
        0.234/65.2 & 
        - \\
        
        AutoDIR & 
        0.247/57.9 & 
        0.315/144.1 & 
        0.105/30.6 & 
        0.181/27.0 & 
        - & 
        0.157/22.2 & 
        0.116/43.7 & 
        0.249/74.0 & 
        0.157/52.4 \\
        \midrule
        
        PromptIR & 
        0.262/62.0 & 
        0.333/150.9 & 
        0.111/49.3 & 
        0.186/29.3 & 
        0.128/15.8 & 
        0.186/32.9 & 
        0.258/111.8 & 
        0.391/99.3 & 
        0.208/106.8 \\
        
        PromptIR GenDS & 
        0.212/56.0 & 
        0.160/89.0 & 
        0.096/34.4 & 
        0.182/28.1 & 
        0.119/13.9 & 
        0.191/31.9 & 
        0.178/87.9 & 
        0.375/90.7 & 
        0.182/79.8 \\
        
        Swin & 
        0.242/62.9 & 
        0.254/109.9 & 
        0.182/38.8 & 
        0.189/27.1 & 
        0.143/21.7 & 
        0.198/31.7 & 
        0.241/112.0 & 
        0.293/88.3 & 
        0.232/82.6 \\
        
        Swin GenDS & 
        0.209/54.3 & 
        0.165/74.6 & 
        0.116/35.8 & 
        0.162/24.1 & 
        0.121/14.1 & 
        0.170/36.2 & 
        0.167/73.1 & 
        0.241/72.1 & 
        0.197/70.7 \\
        
        NAFNet & 
        0.211/71.3 & 
        0.183/99.2 & 
        0.107/34.4 & 
        0.200/29.3 & 
        0.131/14.3 & 
        0.155/28.2 & 
        0.167/78.8 & 
        0.304/83.5 & 
        0.178/73.4 \\
        
        NAFNet GenDS & 
        0.151/52.5 & 
        0.143/76.7 & 
        0.100/31.5 & 
        0.180/27.1 & 
        0.110/11.3 & 
        0.149/28.7 & 
        0.147/63.7 & 
        0.278/78.5 & 
        0.170/60.5 \\
        \bottomrule
    \end{tabularx}
\end{table*}



\begin{table*}[t]
    \centering
    \small
    \begin{tabular}{cccccccccc}
         Method&O-Haze&REVIDE&RainDS syn&LHP&RSVD&GoPro&LOLv1&SICE&Raindrop  \\
         DiffUIR&0.2684/58.53&0.3335/147.15&0.0881/31.17&0.1865/26.48&0.1764/26.14&0.1443/25.16&0.1479/65.10&0.4418/102.88&\\
         
         Diff-Plugin&0.2806/72.93&0.3766/164.69&0.1937/45.03&0.1778/30.22&0.2072/22.49&0.2168/32.82&0.1947/70.46&0.2334/69.23&\\
         
         InstructIR&0.3132/65.38&0.3410/154.47&0.1165/29.24&0.1389/21.21&&0.1460/21.11&0.1324/57.26&0.2341/65.15&\\
         
         AutoDIR&0.2471/57.89&0.3154/144.12&0.1052/30.57& 0.1813/27.01&&0.1566/22.22&0.1157/43.71&0.2489/74.03&0.157/52.37\\
         
         PromptIR&0.2615/62.03&0.3328/150.94&0.1114/49.34&0.1856/29.35&0.1279/15.81&0.1857/32.87&0.2582/111.81&0.3905/99.29&0.2082/106.83\\
         
         PromptIR GenDS&0.2116/55.99&0.1595/88.99&0.0957/34.41&0.1817/28.15&0.1188/13.93&0.1908/31.94&0.1777/87.93&0.3751/90.68&0.1822/79.76\\
         
         Swin&0.2417/62.88&0.2537/109.88&0.182/38.81&0.1891/27.07&0.1209/14.14&0.1984/31.74&0.2407/112.03&0.2928/88.32&0.232/82.58\\
         
         Swin GenDS&0.2089/54.25&0.1652/74.56&0.1160/35.78&0.1620/24.13&0.1209/14.14&0.1699/36.18&0.1670/73.12&0.2408/72.11&0.1974/70.68\\
         
         NAFNet&0.211/71.34&0.183/99.17&0.107/34.35&0.1998/29.33&0.131/14.32&0.1552/28.17&0.1673/78.76&0.304/83.46&0.1779/73.41\\
         
         NAFNet GenDS&0.1512/52.51&0.143/76.69&0.0999/31.47&0.1796/27.09&0.143/21.78&0.1489/28.68&0.1465/63.72&0.2783/78.52&0.1698/60.52
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}



% \begin{table*}[t]
%     \centering
%     \setlength{\tabcolsep}{1pt}
%     \begin{tabular}{c|c|c|c|c|c|c|c}
%         \multirow{3}{*}{Method} &\multicolumn{5}{|c|}{Within Distribution} & \multicolumn{2}{|c}{Out of Distribution} \\ \cline{2-8}
%         &\multicolumn{3}{|c|}{Real}&\multicolumn{2}{|c|}{Synthetic} & \multicolumn{2}{|c}{Real} \\ \hline

%         & Densehaze&NN-Haze&I-Haze&RESIDE&Cityscapes Fog&REVIDE&O-Haze\\ \cline{2-8}
%         DiffUIR&10.20/0.359/0.7989/322.58&12.59/0.498/0.5074/220.10&14.02/0.732/0.2084/135.65&32.94/0.956/0.0129/3.71&18.56/0.834/0.1203/25.28&17.26/0.792/0.2684/58.53&16.59/0.705/0.3335/147.15 \\
%         DiffPlugin&10.54/0.363/0.763/326.64&12.19/0.333/0.5229/237.72&18.36/0.742/0.2034/156.08&23.23/0.765/0.0906/21.40&16.92/0.728/0.1784/28.77&17.45/0.728/0.2806/72.93&15.79/0.471/0.3766/164.69 \\
%         InstructIR&10.52/0.436/0.7585/336.47&12.52/0.502/0.5111/243.45&16.05/0.777/0.3276/176.45&26.90/0.952/0.0169/5.62&16.42/0.791/0.1607/32.08&16.51/0.831/0.3132/65.38&16.56/0.709/0.3410/154.47 \\
%         AutoDIR&11.69/0.381/0.770/310.78&13.00/0.519/0.4829/218.52&16.86/0.814/0.1675/125.15&30.98/0.974/0.0132/3.811&19.04/0.846/0.100/23.12&16.31/0.782/0.2471/57.89&17.57/0.731/0.3154/144.12 \\
%         PromptIR base&11.11/0.376/0.7888/328.71&12.62/0.494/0.5132/221.45&17.36/0.806/0.1914/143.74&29.13/0.967/0.0159/5.28&28.10/0.961/0.0393/6.08&17.56/0.786/0.2615/62.03&16.46/0.701/0.3328/150.94\\
%         PromptIR fulldata res&16.25/0.490/0.5612/312.94&16.07/0.668/0.3105/138.88&20.07/0.857/0.1291/99.44&30.87/0.977/0.0136/5.14&29.08/0.964/0.0382/6.34&19.20/0.827/0.2116/55.99&22.40/0.849/0.1595/88.99\\

%         NAFNet res&16.99/0.5165/0.518/327.77&18.11/0.714/0.276/152.80&21.33/0.867/0.127/104.00&32.31/0.981/0.0108/3.26&33.40/0.979/0.0207/3.302&18.71/0.819/0.211/71.34&19.85/0.814/0.183/99.17\\

%         NAFnet fulldata res&17.67/0.545/0.4736/316.06&19.10/0.743/0.2421/109.51&20.57/0.869/0.1088/89.96&34.80/0.986/0.0075/2.88&32.55/0.977/0.0244/3.76&20.96/0.871/0.1512/52.51&20.51/0.849/0.143/76.69\\
        
%         Swin e44 origdata&16.24/0.458/0.6470/332.5&16.49/0.635/0.3858/172.37&21.87/0.874/0.135/95.23&36.16/0.987/0.0083/2.956&28.62/0.956/0.0437/6.568&18.44/0.812/0.2417/62.88&20.12/0.802/0.2537/109.88\\
%         Swin fulldata&17.90/0.530/0.5158/315.05&20.31/0.742/0.2506/117.14&22.05/0.883/0.1099/87.39&38.08/0.989/0.0067/2.81&33.45/0.972/0.0270/3.82&18.69/0.831/0.2089/54.25&20.60/0.843/0.1652/74.56\\
%     \end{tabular}
%     \caption{Haze}
%     \label{tab:my_label}
% \end{table*}


% \begin{table*}[t]
%     \centering
%     \setlength{\tabcolsep}{1pt}
%     \begin{tabular}{c|c|c|c|c|c|c|c|c}
%         \multirow{3}{*}{Method} &\multicolumn{6}{|c|}{Within Distribution} & \multicolumn{2}{|c}{Out of Distribution} \\ \cline{2-9}
%         &\multicolumn{2}{|c|}{Real}&\multicolumn{4}{|c|}{Synthetic} &\multicolumn{1}{|c}{Synthetic}& \multicolumn{1}{|c}{Real} \\ \hline
        
%         & RainDS&RealRain1k&ORD&Rain 13K&Rain1400&SPAC&RainDS&LHP\\ \cline{2-9}
        
%         DiffUIR &25.70/0.802/0.1445/49.36&27.02/0.905/0.0882/18.23&16.82/0.644/0.3852/143.16&31.03/0.904/0.0689/14.10&27.76/0.899/0.1414/42.54&23.70/0.803/0.2231/53.81&30.85/0.897/0.0881/31.17&26.71/0.832/0.1865/26.48 \\
%         DiffPlugin&21.39/0.526/0.2153/60.65&24.14/0.660/0.1503/35.00&13.39/0.470/0.4225/94.62&21.71/0.617/0.1689/26.86&22.27/0.623/0.1549/46.61&24.46/0.733/0.1180/18.86&22.04/0.635/0.1937/45.03&26.02/0.735/0.1778/30.22 \\
%         InstructIR-7D&25.41/0.789/0.1506/51.93&30.71/0.939/0.0668/16.70&13.37/0.565/0.4360/89.21&29.56/0.885/0.0879/16.06&30.97/0.907/0.0705/25.09&31.97/0.951/0.0553/11.23&30.24/0.879/0.1165/29.24&28.93/0.871/0.1389/21.21\\
%         AutoDIR&24.87/0.773/0.1606/69.21&30.04/0.924/0.0794/18.21&14.29/0.594/0.3935/93.56&30.52/0.895/0.073/12.65&31.18/0.913/0.055/17.64&31.69/0.941/0.0768/17.49&29.14/0.858/0.1052/30.57& 28.44/0.841/0.1813/27.01\\
%         PromptIR base&24.28/0.759/0.1569/75.87&32.85/0.922/0.0949/19.47&25.53/0.863/0.1244/47.54&29.85/0.884/0.0892/17.45&30.69/0.901/0.0731/26.23&33.07/0.958/0.0450/9.14&29.70/0.871/0.1114/49.34&25.85/0.835/0.1856/29.35\\
%         PromptIR fulldata res&25.36/0.788/0.1352/50.35&32.02/0.917/0.1027/19.54&26.45/0.866/0.1346/48.05&30.17/0.888/0.0101/18.41&31.11/0.908/0.0716/24.82&34.32/0.964/0.0297/6.54&30.00/0.884/0.0957/34.41&26.15/0.840/0.1817/28.15\\


%         NAFNet res&25.73/0.798/0.134/45.92&34.98/0.951/0.0554/14.71&29.18/0.896/0.0891/29.65&31.22/0.904/0.078/14.48&31.73/0.917/0.0633/21.36&34.59/0.966/0.0257/4.94&28.49/0.887/0.107/34.35&27.41/0.835/0.1998/29.33\\

%         NAFNet fulldata res&25.94/0.800/0.1297/41.22&34.28/0.947/0.0594/14.46&29.02/0.893/0.1041/33.43&31.23/0.906/0.0792/15.22&31.56/0.916/0.0661/22.80&34.78/0.967/0.0288/5.66&30.40/0.891/0.0999/31.47&27.53/0.848/0.1796/27.09\\

%         Swin e44 origdata&25.63/0.793/0.151/47.098&33.26/0.936/0.0649/14.47&27.39/0.859/0.1501/39.30&30.89/0.898/0.0850/15.837&31.16/0.909/0.0702/23.711&33.82/0.959/0.0314/6.619&28.50/0.863/0.182/38.81&28.97/0.863/0.1891/27.07\\

%          Swin fulldata&25.97/0.794/0.1494/46.46&34.15/0.951/0.0535/13.25&28.31/0.867/0.1340/36.88&30.62/0.894/0.0980/17.96&30.98/0.907/0.0710/25.07&33.37/0.957/0.0365/7.29&29.34/0.868/0.1160/35.78&29.30/0.869/0.1620/24.13\\

%          Swin synthetic&24.84/0.755/0.2200/77.44&30.68/0.927/0.0782/16.52&22.92/0.734/0.3148/96.16&27.98/0.834/0.1857/32.85&28.16/0.848/0.1594/52.78&31.26/0.926/0.0969/21.86&27.63/0.807/0.2202/69.96&27.87/0.843/0.2076/26.84\\
        
%     \end{tabular}
%     \caption{Rain}
%     \label{tab:my_label}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     \begin{tabular}{c|c|c|c|c}
%         \multirow{3}{*}{Method} &\multicolumn{3}{|c|}{Within Distribution} & \multicolumn{1}{|c}{Out of Distribution} \\ \cline{2-5}
%         &\multicolumn{3}{|c|}{Synthetic} & \multicolumn{1}{|c}{Synthetic} \\ \hline

%         & Cityscapes Snow&CSD&Snow100k&RSVD\\ \hline
%         DiffUIR&12.42/0.330/0.5825/20.16&17.57/0.790/0.1962/43.81&28.76/0.869/0.1379/7.05&21.60/0.823/0.1764/26.14\\
%         DiffPlugin&22.25/0.694/0.2420/35.35&15.61/0.635/0.2431/41.14&21.02/0.611/0.1960/4.10&18.92/0.662/0.2072/22.49 \\

%         PromptIR base&30.16/0.918/0.1089/26.31&27.62/0.919/0.0708/23.34&27.86/0.863/0.1204/5.39&20.08/0.838/0.1279/15.81\\
%         PromptIR fulldata res&31.44/0.934/0.0886/19.73&28.03/0.920/0.0702/23.92&28.51/0.874/0.1148/4.92&21.77/0.858/0.1188/13.93\\


%         NAFNet res&33.67/0.953/0.0627/7.23&31.92/0.947/0.044/14.13&30.01/0.893/0.0961/3.25&21.32/0.848/0.131/14.32\\

%         NAFNet fulldata res&33.02/0.950/0.0608/6.96&31.39/0.942/0.0484/15.36&29.78/0.891/0.0997/3.38&22.81/0.873/0.1106/11.33\\
%         Swin e44 origdata&32.38/0.934/0.0812/9.41&32.01/0.935/0.0577/19.131&29.34/0.880/0.1035/3.871&22.05/0.838/0.143/21.78\\

%         Swin fulldata&32.17/0.929/0.0849/9.46&31.95/0.933/0.0592/20.52&29.23/0.881/0.1073/4.34&23.07/0.863/0.1209/14.14\\

%         Swin synthetic&27.09/0.864/0.1587/29.24&27.53/0.869/0.1706/48.46&25.63/0.808/0.2122/10.58&22.98/0.844/0.1726/21.80\\
%     \end{tabular}
%     \caption{Snow}
%     \label{tab:my_label}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     \begin{tabular}{c|c|c|c|c}
%         \multirow{3}{*}{Method} &\multicolumn{3}{|c|}{Within Distribution} & \multicolumn{1}{|c}{Out of Distribution} \\ \cline{2-5}
%         &\multicolumn{3}{|c|}{Real} & \multicolumn{1}{|c}{Real} \\ \hline

%         & HIDE&RealBlur&REDS&GoPro\\ \hline
%         DiffUIR&27.17/0.854/0.1741/26.23&26.15/0.721/0.1881/44.80&26.84/0.825/0.1851/57.64&29.17/0.864/0.1443/25.16 \\
%         DiffPlugin&21.40/0.658/0.2468/39.68&23.62/0.728/0.1920/43.65&21.47/0.628/0.2158/68.40&21.76/0.633/0.2168/32.82 \\
%         InstructIR&27.50/0.859/0.1647/21.37&27.09/0.845/0.1269/25.39&26.93/0.831/0.1544/48.82&28.26/0.870/0.1460/21.11 \\
%         AutoDIR&27.03/0.862/0.1697/21.67&24.77/0.770/0.1486/28.58&27.23/0.846/0.1669/49.77&27.07/0.828/0.1566/22.22 \\
%         OneRestore&/&/&/&/\\
%         MaskRestore&/&/&/&28.02/0.859\\
%         PromptIR base&26.55/0.837/0.1904/30.07&28.13/0.845/0.1682/35.78&29.45/0.867/0.1328/41.52&26.98/0.828/0.1857/32.87 \\
%         PromptIR fulldata res&26.70/0.845/0.2042/30.29&28.44/0.857/0.1654/32.81&29.58/0.871/0.1455/41.70&27.28/0.843/0.1908/31.94\\
%         NAFNet res&27.40/0.864/0.164/25.66&28.93/0.876/0.1396/27.41&30.94/0.898/0.1046/33.10&28.14/0.868/0.1552/28.17\\
%         NAFNet fulldata res&27.53/0.866/0.1630/26.68&29.03/0.879/0.1380/27.68&30.82/0.896/0.1096/33.59&27.80/0.864/0.1489/28.68\\
%         Swin e44 origdata&25.91/0.829/0.226/34.35&28.15/0.851/0.1823/39.60&29.23/0.866/0.1761/48.14&26.79/0.843/0.1984/31.74\\
%         Swin fulldata&25.89/0.830/0.1960/34.24&22.74/0.739/0.2283/48.39&29.01/0.866/0.1448/43.88&26.09/0.830/0.1699/36.18\\

%         Swin synthetic&25.36/0.804/0.2247/37.20&27.24/0.813/0.1474/34.83& 28.49/0.849/0.1498/47.06&25.70/0.814/0.1807/34.71\\
        
%     \end{tabular}
%     \caption{Motion blur}
%     \label{tab:my_label}
% \end{table*}


% \begin{table*}[t]
%     \centering
%     \begin{tabular}{c|c|c|c|c}
%         \multirow{3}{*}{Method} &\multicolumn{2}{|c|}{Within Distribution} & \multicolumn{2}{|c}{Out of Distribution} \\ \cline{2-5}
%         &\multicolumn{2}{|c|}{Real} & \multicolumn{2}{|c}{Real} \\ \hline

%         & LOLv2&SID&LOLv1&SICE\\ \hline
%         PromptIR&/&/&/&/ \\
%         TextualDeg&/&/&/&/ \\
%         DiffUIR&20.27/0.826/0.2039/64.17&9.86/0.061/0.8987/456.35&21.65/0.836/0.1479/65.10&10.00/0.367/0.4418/102.88 \\
%         DiffPlugin&18.00/0.644/0.2263/62.83&12.47/0.365/0.7028/298.52&19.38/0.713/0.1947/70.46&17.59/0.611/0.2334/69.23 \\
%         InstructIR&23.99/0.857/0.1562/46.28&12.84/0.377/0.6491/269.21&22.81/0.836/0.1324/57.26&17.58/0.750/0.2341/65.15 \\
%         AutoDIR&19.94/0.800/0.1759/48.02&13.45/0.457/0.6650/262.27&22.37/0.888, 20.53/0.850/0.1157/43.71&15.37/0.685/0.2489/74.03 \\
%         OneRestore&/&/&/&/\\
%         MaskRestore&/&/&24.46/0.858&/\\
%         PromptIR base&17.25/0.710/0.2642/76.65&17.67/0.517/0.5781/303.10&20.53/0.768/0.2582/111.81&12.42/0.438/0.3905/99.29\\
%         PromptIR fulldata res&21.90/0.868/0.1422/51.75&18.31/0.550/0.5661/285.43&21.38/0.812/0.1777/87.93&11.41/0.466/0.3751/90.68\\
%         NAFNet res&22.54/0.866/0.140/49.89&18.13/0.557/0.558/294.83&22.37/0.826/0.1673/78.76&14.03/0.592/0.304/83.46\\

%         NAFNet fulldata res&22.87/0.887/0.1195/38.55&18.64/0.586/0.5143/258.75&22.82/0.838/0.1465/63.72&14.65/0.614/0.2783/78.52\\

%         Swin e44 origdata&21.97/0.844/0.1954/70.92&17.12/0.517/0.6465/304.38&20.07/0.784/0.2407/112.03&15.27/0.667/0.2928/88.32\\

%         Swin fulldata&22.32/0.869/0.1458/49.53&16.18/0.483/0.5905/282.73&24.27/0.842/0.1670/73.12&16.05/0.678/0.2408/72.11 \\

%         Swin synthetic&19.19/0.778/0.2303/69.01&15.02/0.487/0.6995/287.45&17.35/0.743/0.2516/96.85&14.84/0.626/0.2912/81.32\\
%     \end{tabular}
%     \caption{Low-light}
%     \label{tab:my_label}
% \end{table*}

% \begin{table*}[t]
%     \centering
%     \begin{tabular}{c|c|c|c}
%         \multirow{3}{*}{Method} &\multicolumn{2}{|c|}{Within Distribution} & \multicolumn{1}{|c}{Out of Distribution} \\ \cline{2-4}
%         &\multicolumn{1}{|c|}{Real}&\multicolumn{1}{|c|}{Synthetic} & \multicolumn{1}{|c}{Real} \\ \hline

%         & Raindrop&RainDS&RainDS\\
%         AutoDIR&30.10/0.924/0.0583/25.53&20.22/0.795/0.3327/110.66&23.33/0.754/0.157/52.37 \\
%         OneRestore&/&/&/ \\
%         MaskRestore&/&/&/\\
%         PromptIR base&27.04/0.885/0.1197/80.07&21.76/0.852/0.2589/88.90&20.94/0.709/0.2082/106.83\\
%         PromptIR fulldata res&29.15/0.908/0.0710/45.40&20.91/0.829/0.3054/103.91&22.04/0.718/0.1822/79.76\\
%         NAFNet res&29.61/0.914/0.083/48.30&28.23/0.924/0.088/31.52&22.91/0.745/0.1779/73.41\\
%         NAFNet fulldata res&30.33/0.922/0.0557/30.42&28.26/0.927/0.0838/29.43&23.31/0.747/0.1698/60.52\\
%         Swin e44 origdata&28.74/0.903/0.0894/53.30&26.98/0.893/0.1053/40.88&22.34/0.726/0.232/82.58\\
%         Swin fulldata&28.89/0.901/0.0812/42.54&26.87/0.893/0.1035/36.72&22.87/0.740/0.1974/70.68\\
%         Swin synthetic&28.16/0.899/0.0754/44.47&20.95/0.812/0.3043/100.80&20.86/0.706/0.2091/98.53\\
%     \end{tabular}
%     \caption{Raindrop}
%     \label{tab:my_label}
% \end{table*}

==> sec/comments.tex <==
\section{intro}



%On the other hand, other low-level vision tasks such as segmentation and depth estimation have recently combined large scale datasets with simple model architectures to produce foundation models such as SAM and Depth-Anything which achieved significant improvements in zero-shot out-of-distribution performance. For image restoration, we hypothesize that lack of generalization is due to the lack of following datasets: 1. Large-scale datasets with diverse enough scenes 2. Variety of degradation patterns type in a single dataset 3. Same clean image under different degradations in a single dataset. We now elaborate each of these reasons and their effect on generalizable image restoration models. 

% Recent advancements in the field of foundation models such as SAM, Depth-Anything and CLIP can be greatly attributed to the amount of data being used to train such models. This large-scale data allows the model to generalize to various scenes enabling real-world applications. For instance, CLIp was trained on $300M$ image-text pairs. In contrast, most image restoration datasets that are used to train current all-in-one models rarely exceed $10,000$ samples as shown in Table. Furthermore, some datasets such as RESIDE containing $72,135$ clean-degraded pairs are produced from the same set of approximately $2000$ clean images. This can cause existing models to over-fit to the scenes present in the dataset. Thus, larger datasets with more diverse scenes would improve generalization. 

% Moreover, many existing restoration datasets are synthetic and are typically governed by a single model. Thus, training a network on one such dataset for a single degradation can cause it to overfit to the degradation patterns of that model. This can cause the performance to suffer in real-world conditions as the same dergadation can occur in different patterns. A solution for this problem is to collect real-world data or generate data for degradations with a variety of models. However, this is cumbersome and not feasible for some degradations. For instance, it is quite challenging to obtain real degraded images for degradation such as haze and low-light as haze requires the scene to not change for a long time and low-light images need to be captured by specialized cameras. This problem is also tied to first one. needs some elaboration

% Finally, the third issue prevents learning of an degradation-agnostic restoration network. A degradation-agnostic network would be insensitive to the domain or type of degradation present in the image allowing it to work for  out-of-distribution samples. A straightforward appraoch to learning such a degradation-agnostic network would be to extract the same clean features irrespective of whether an image of a particular scene is under different degradations. However, to train such an appraoch, a dataset consisting of a single scene under multiple degradations needs to be used. However, to the best of our knowledge, there is no such dataset at present.

%Thus, datasets for these degradations are typically small unless they are synthetic. However, synthetic data relies on a specific model which may not approximate the real world conditions well enough, causing the model to perform poorly for that degradation if its different from the model. 

% In this paper, we aim to develop a robust all-in-one restoration model capable of generalizing to out-of-distribution restoration by addressing the afore-mentioned issues. Throughout this paper, we define out-of-distribution as the same training degradation types, but the data for testing is taken from a different dataset than training. To address the first issue, we collect a dataset of $1,20,000$ unique clean images by combining over $20$ existing restoration datasets of different degradations. To address the second and third problem, we propose to use generative models to learn the characteristics of various degradations and synthesize multiple degraded versions of a single clean image. Specifically, we train the InstructPix2pix diffusion model with text prompts and condition on a clean image to produce the same clean image under different degradations. Furthermore, we train our diffusion model on a variety of datasets for a single degradation to ensure that it does not heavily rely on a specific degradation model. We then generate a large dataset of $x$ images from the $1,20,000$ clean images using our diffusion model. Finally, we train a foundation model for image restoration dubbed x using contrastive loss for degradation-invariant image restoration. extensive experiments demonstrate that our model achieves state-of-the-art performance and generalization to out-of-distribution datasets. 

Haze {'DiffUIR': 0.32958, 'DiffPlugin': 0.35166000000000003, 'InstructIR': 0.35496, 'AutoDIR': 0.30672, 'PromptIR': 0.30972, 'PromptIR GenDS': 0.21051999999999998, 'NAFNet': 0.19050000000000003, 'NAFNet GenDS': 0.17128, 'Swin': 0.24396, 'Swin GenDS': 0.182}

Rain {'DiffUIR': 0.17521666666666666, 'DiffPlugin': 0.20498333333333338, 'InstructIR': 0.14451666666666665, 'AutoDIR': 0.13971666666666666, 'PromptIR': 0.09725, 'PromptIR GenDS': 0.08065, 'NAFNet': 0.07425000000000001, 'NAFNet GenDS': 0.07788333333333333, 'Swin': 0.0921, 'Swin GenDS': 0.09039999999999998}


Snow {'DiffUIR': 0.3055333333333334, 'DiffPlugin': 0.22703333333333334, 'PromptIR': 0.10003333333333332, 'PromptIR GenDS': 0.0912, 'NAFNet': 0.06760000000000001, 'NAFNet GenDS': 0.06963333333333332, 'Swin': 0.0808, 'Swin GenDS': 0.0838}


Motion blur {'DiffUIR': 0.1824333333333333, 'DiffPlugin': 0.21819999999999998, 'InstructIR': 0.1486666666666667, 'AutoDIR': 0.16173333333333334, 'PromptIR': 0.16380000000000003, 'PromptIR GenDS': 0.1717, 'NAFNet': 0.13606666666666667, 'NAFNet GenDS': 0.1368666666666667, 'Swin': 0.1948, 'Swin GenDS': 0.1897}


Raindrop {'AutoDIR': 0.1955, 'PromptIR': 0.18930000000000002, 'PromptIR GenDS': 0.1882, 'NAFNet': 0.08549999999999999, 'NAFNet GenDS': 0.06975, 'Swin': 0.09734999999999999, 'Swin GenDS': 0.09234999999999999}


Low-light {'DiffUIR': 0.5513, 'DiffPlugin': 0.46455, 'InstructIR': 0.40265, 'AutoDIR': 0.42045, 'PromptIR': 0.42114999999999997, 'PromptIR GenDS': 0.35415, 'NAFNet': 0.34900000000000003, 'NAFNet GenDS': 0.31689999999999996, 'Swin': 0.42095, 'Swin GenDS': 0.36815000000000003}





Haze {'DiffUIR': 0.32958, 'DiffPlugin': 0.35166000000000003, 'InstructIR': 0.35496, 'AutoDIR': 0.30672, 'PromptIR': 0.30972, 'PromptIR GenDS': 0.21051999999999998, 'NAFNet': 0.19050000000000003, 'NAFNet GenDS': 0.17128, 'Swin': 0.24396, 'Swin GenDS': 0.182}



Rain {'DiffUIR': 0.17521666666666666, 'DiffPlugin': 0.20498333333333338, 'InstructIR': 0.14451666666666665, 'AutoDIR': 0.13971666666666666, 'PromptIR': 0.09725, 'PromptIR GenDS': 0.08065, 'NAFNet': 0.07425000000000001, 'NAFNet GenDS': 0.07788333333333333, 'Swin': 0.0921, 'Swin GenDS': 0.09039999999999998}



Snow {'DiffUIR': 0.3055333333333334, 'DiffPlugin': 0.22703333333333334, 'PromptIR': 0.10003333333333332, 'PromptIR GenDS': 0.0912, 'NAFNet': 0.06760000000000001, 'NAFNet GenDS': 0.06963333333333332, 'Swin': 0.0808, 'Swin GenDS': 0.0838}



Motion blur {'DiffUIR': 0.1824333333333333, 'DiffPlugin': 0.21819999999999998, 'InstructIR': 0.1486666666666667, 'AutoDIR': 0.16173333333333334, 'PromptIR': 0.16380000000000003, 'PromptIR GenDS': 0.1717, 'NAFNet': 0.13606666666666667, 'NAFNet GenDS': 0.1368666666666667, 'Swin': 0.1948, 'Swin GenDS': 0.1897}


Raindrop {'AutoDIR': 0.1955, 'PromptIR': 0.18930000000000002, 'PromptIR GenDS': 0.1882, 'NAFNet': 0.08549999999999999, 'NAFNet GenDS': 0.06975, 'Swin': 0.09734999999999999, 'Swin GenDS': 0.09234999999999999}


Low-light {'DiffUIR': 0.5513, 'DiffPlugin': 0.46455, 'InstructIR': 0.40265, 'AutoDIR': 0.42045, 'PromptIR': 0.42114999999999997, 'PromptIR GenDS': 0.35415, 'NAFNet': 0.34900000000000003, 'NAFNet GenDS': 0.31689999999999996, 'Swin': 0.42095, 'Swin GenDS': 0.36815000000000003}



% \begin{table*}
% \begin{center}
% \resizebox{1.8\columnwidth}{!}{
% \begin{tabular}
% {@{\extracolsep{4pt}}c c c c c c c c c c@{}}
% \toprule
%  & & \multicolumn{4}{c}{ActivityNet \cite{activitynet}} & \multicolumn{4}{c}{Charades STA \cite{charades}} \\
% \cline{3-6} \cline{7-10} \\
% Method & Extra Training Data & mR@1 (\(\uparrow\)) & mR@5 (\(\uparrow\)) & mAP (\(\uparrow\)) & mIoU  (\(\uparrow\)) & mR@1 
% (\(\uparrow\)) & mR@5 (\(\uparrow\)) & mAP (\(\uparrow\)) & mIoU (\(\uparrow\))\\
% \midrule
% % CM2 &  \\
% %\color{blue} Existing MR methods\\
% VideoChatGPT-7B \cite{videochatgpt} & 0.1M & 15.36 & - & - & 18.9 & 9.8 & - & - & 13.7\\
% VTimeLLM-7B \cite{vtimellm}& 0.7M & 28.7 & - & - & 30.4 & 29.97 & - & - & 31.2 \\
% VTimeLLM-13B \cite{vtimellm}& 0.7M & \underline{29.5} & - & - & \underline{31.4} & 34.77 & - & - & \underline{34.6} \\
% UniVTG (0-shot) \cite{univtg}& 4.2M & 13.16 & 24.50 & 7.04 & 17.19 & 29.81 & \underline{58.53} & 21.73 & 29.77\\
% UniVTG (tuned) \cite{univtg}& 4.2M & \textbf{40.73} & \textbf{61.43} & \textbf{27.53} & \textbf{40.37} & \textbf{55.99} & \textbf{62.52} & \textbf{35.68} & \textbf{51.25}\\

% \midrule
% Ours & - & 24.5 & \underline{49.62} & \underline{18.9} & 27.27 & \underline{35.09} & 54.84 & \underline{24.79} & 34.5\\

% \bottomrule
% \end{tabular}}
% \caption{Comparison of our method against existing MR methods. While our method does not surpass SOTA techniques, it demonstrates promising results and occasionally even outperforms LLM-based methods. This is particularly notable given that SOTA methods typically rely on LLMs or large amounts of pre-training data. In contrast, our approach does not require dedicated MR training and utilizes a simple text-matching technique for inference, leaving ample room for improvement. Bold - highest, underline - second highest}
% % \caption{Comparison of our method against existing MR methods. Although our method is inferior to SOTA methods, it shows promising results, sometimes even outperforming LLM-based methods, especially considering that SOTA methods either rely on LLMs or leverage extensive amounts of pre-training data. In contrast, our approach does not require dedicated MR training and utilizes a simple text-matching technique for inference, leaving ample room for improvement. Bold - highest, underline - second highest}
% \vskip-8pt
% \label{mr_table}
% \end{center}
% \end{table*}
